Jolteon and Ditto: Network-Adaptive Efficient Consensus with Asynchronous Fallback

Existing committee-based Byzantine state machine replication (SMR) protocols, typically deployed in production blockchains, face a clear trade-off: (1) they either achieve linear communication cost in the happy path, but sacrifice liveness during periods of asynchrony, or (2) they are robust (progress with probability one) but pay quadratic communication cost. We believe this trade-off is unwarranted since existing linear protocols still have asymptotic quadratic cost in the worst case. We design Ditto, a Byzantine SMR protocol that enjoys the best of both worlds: optimal communication on and off the happy path (linear and quadratic, respectively) and progress guarantee under asynchrony and DDoS attacks. We achieve this by replacing the view-synchronization of partially synchronous protocols with an asynchronous fallback mechanism at no extra asymptotic cost. Specifically, we start from HotStuff, a state-of-the-art linear protocol, and gradually build Ditto. As a separate contribution and an intermediate step, we design a 2-chain version of HotStuff, Jolteon, which leverages a quadratic view-change mechanism to reduce the latency of the standard 3-chain HotStuff. We implement and experimentally evaluate all our systems. Notably, Jolteon's commit latency outperforms HotStuff by 200-300ms with varying system size. Additionally, Ditto adapts to the network and provides better performance than Jolteon under faulty conditions and better performance than VABA (a state-of-the-art asynchronous protocol) under faultless conditions. This proves our case that breaking the robustness-efficiency trade-off is in the realm of practicality.

==> sections/2-chain.tex <==
\section{Get $2$-chain Commit for Free}\label{app:2-chain}

\lef{Shouldn't we already have this integrated in section 4?}

In this section, we show how to slightly modify the $3$-chain commit protocol in Figure~\ref{fig:fallback_protocol} into a $2$-chain commit protocol, strictly improving the commit latency without losing any of the nice guarantees.
Earlier solutions that can be adapted into the chain-based BFT SMR framework with $2$-chain commit either pay a quadratic cost for the view-change~\cite{castro1999practical, jalalzai2020fast}, or sacrifices responsiveness (cannot proceed with network speed)~\cite{buchman2016tendermint, buterin2017casper, yin2019hotstuff}.
Since our protocol already pays the quadratic cost, which is inevitable for the asynchronous view-change~\cite{abraham2019asymptotically}, we can get the improvement over the commit latency of the protocol from $3$-chain commit ($6$ rounds) to $2$-chain commit ($4$ rounds), without sacrificing anything else.


The difference compared with the protocol in Figure~\ref{fig:fallback_protocol} with $3$-chain commit is marked red in Figure~\ref{fig:2-chain}.
Intuitively, $2$-chain commit means the protocol only needs two adjacent certified blocks in the same view to commit the first block, and to ensure safety, now replicas lock on the highest QC's rank ($1$-chain lock) instead of the parent QC's rank of the highest QC.
Moreover, since now a block can be committed with $2$-chain, the asynchronous fallback only needs every replica to build a fallback-chain of $2$ fallback-blocks instead of $3$, to ensure progress made during the fallback.
Hence, $2$ rounds can be reduced during the fallback if the protocol uses a $2$-chain commit.
Another main difference is that, with $2$-chain commit and $1$-chain lock, only one honest replica $h$ may have the highest QC among all honest replicas when entering the asynchronous fallback. Then, only the fallback-chain proposed by $h$ will get $2f+1$ votes from all honest replica and be completed, while other f-chains proposed by other honest replica extending a lower-ranked QC may not get $2f+1$ votes, since $h$ will not vote due to the $1$-chain locking.
A straightforward solution is to allow replicas to adopt f-chains from other replicas, and build their f-chains on top of the first certified f-chain they know.
% This is similar to the optimization technique we discussed in Section~\ref{sec:fallback} for practical performance, and here it is crucial to guarantee the liveness of the protocol.
With the changes above, even if only one fallback-chain is live, all honest replicas can complete their fallback-chain and ensure the liveness of the asynchronous fallback.







To summarize, the $2$-chain-commit version of the protocol strictly improves the latency of the $3$-chain commit version, by reducing the commit latency by $2$ rounds for both Steady State and Asynchronous Fallback.
The correctness proof of the $2$-chain commit protocol would be analogous to that for the $3$-chain commit version, and we omit it here for brevity.

==> sections/2chain-VABA.tex <==
% \paragraph{2-chain VABA:}
% As a by-product of \async, we can improve the latency of VABA~\cite{abraham2019asymptotically} from expected $16.5$ rounds to expected $10.5$ rounds, through chaining and pipelining. We refer to the improved version of VABA as \vaba and the analysis can be found in Appendix~\ref{app:TODO}.
% We obtain our \vaba protocol, by simply disabling the synchronous path of \async.
% More specifically, \vaba is obtained by setting the timeout \timeoutvalue to $0$ in \async (Figure~\ref{fig:steady-state} and \ref{fig:fallback-protocol}). 
% Then, whenever the replica enters a new view, it immediately enters the fallback carrying its highest QC for the new view. Therefore, the synchronous path is never executed, and the exchange of \timeout messages acts as the view-change phase in the original VABA~\cite{abraham2019asymptotically}.
% The correctness of \vaba can be implied by the correctness of \async, as \async is safe and live under asynchrony.


\section{\vaba Details}
\label{sec:vaba}
The original VABA~\cite{abraham2019asymptotically} is designed for single-shot value, runs in views, and each view consists of a leader nomination phase, a leader election phase and a view-change phase. 
The leader nomination phase uses $n$ parallel instances of $3$-chain HotStuff (with each replica as the stable leader) to broadcast and certify its value. This phase takes $4$ RTTs or $8$ rounds, because intuitively $3$-chain commit needs $3$ RTTs to commit a value and $1$ extra RTT to ensure every replica receives the commit proofs.
Then every replica exchanges the proofs showing the leader nomination phase has finished, and runs the leader election phase to decide which replica's value to commit. 
Finally, during view-change phase replicas exchange their local information about the elected leader's value, to ensure safety for entering the next view if no value is committed. With probability $2/3$, each view of VABA will succeed and consensus is reached.
Therefore, the latency of VABA is $(8+1+1+1)\times 1.5=16.5$ rounds in expectation.

VABA can be easily turned into a chained BFT SMR protocol, by having $3$-chain HotStuff instances building chained blocks instead of just values during the leader nomination phase. As a result, the number of blocks to certify is $4$ for each replica's VABA chain.
However, as we shown in our asynchronous fallback protocol (Figure~\ref{fig:fallback-protocol}), the number of blocks can be reduced to just $2$, by the following observations:
(1) We adopt $2$-chain commit instead of $3$-chain commit, and thus immediately reducing the latency by 1 RTT;
(2) We observe the one extra RTT during the leader nomination phase for exchanging commit proofs is unnecessary once we have chained blocks, as the information is embedded in the blockchain and replicas can learn the commit from the chain.
Therefore, we are able to reduce the latency of each view by $4$ rounds ($2$ RTTs), and since the expected number of views VABA needs to execute is $3/2$, the reduced latency is $4\times 3/2=6$ rounds.


==> sections/experiments/2chain.tex <==
\section{No faults Merge these into one}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/3chain-latency}
    \caption{Latency-throughput graph of 3-chain HotStuff for various committee sized. The transaction and batch sizes are set to 512B and 500KB respectively.}
    \label{fig:3chain-latency}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/2chain-latency}
    \caption{Latency-throughput graph of 2-chain HotStuff for various committee sized. The transaction and batch sizes are set to 512B and 500KB respectively.}
    \label{fig:2chain-latency}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/sync-latency}
    \caption{Latency-throughput graph of the sync path for various committee sized. The transaction size is set to 512 B, and the batch size varies from 200 to 1,000 transactions.}
    \label{fig:2chain-latency}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vaba-latency}
    \caption{Latency-throughput graph of 2-chain VABA for various committee sized. The transaction size is set to 512 B, and the batch size is 1,000 transactions.}
    \label{fig:3chain-latency}
\end{figure}

\clearpage

\section{Leader Under Attack Merge into One and add \sync and Hotstuff line at zero}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/async-latency}
    \caption{Latency-throughput graph of Async Fallback for various committee sized. 
    %The transaction size is set to 512 B, and the batch size is 1,000 transactions.
    }
    \label{fig:3chain-latency}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vaba-latency}
    \caption{Latency-throughput graph of 2-chain VABA for various committee sized. The transaction size is set to 512 B, and the batch size is 1,000 transactions.}
    \label{fig:3chain-latency}
\end{figure}

\clearpage

\section{Random Faults Merge Into One}
\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/3chain-faults-latency}
    \caption{Latency-throughput graph of 3-chain HotStuff for 1 and 3 faulty (dead) nodes. The transaction and batch sizes are set to 512B and 500KB respectively. The consensus timeout delay is set to 5 seconds.}
    \label{fig:3chain-faults-latency}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/2chain-faults-latency}
    \caption{Latency-throughput graph of 2-chain HotStuff for 1 and 3 faulty (dead) nodes. The transaction and batch sizes are set to 512B and 500KB respectively. The consensus timeout delay is set to 5 seconds.}
    \label{fig:2chain-faults-latency}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/sync-faults-latency}
    \caption{Latency-throughput graph of sync path for 1 and 3 faulty (dead) nodes. The transaction and batch sizes are set to 512B and 500KB respectively. The consensus timeout delay is set to 5 seconds.}
    \label{fig:3chain-faults-latency}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vaba-faults-latency}
    \caption{Latency-throughput graph of vaba for 1 and 3 faulty (dead) nodes. The transaction sizes are set to 512B.}
    \label{fig:3chain-faults-latency}
\end{figure}

\clearpage
\section{Random Faults with Leader under Attack Merge Into One and add \sync and Hotstuff  line at zero}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/async-faults-latency}
    \caption{Latency-throughput graph of async path for 1 and 3 faulty (dead) nodes. The transaction sizes are set to 512B.}
    \label{fig:3chain-faults-latency}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.47\textwidth]{figures/vaba-faults-latency}
    \caption{Latency-throughput graph of vaba for 1 and 3 faulty (dead) nodes. The transaction sizes are set to 512B.}
    \label{fig:3chain-faults-latency}
\end{figure}

==> sections/experiments/3chain.tex <==
%-------------------------------------------------------------------------------
\subsection{Micro-Benchmarks}
%-------------------------------------------------------------------------------


Add graphs with block commit latency for \sync, Hotstuff, \async with and without faults.
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.47\textwidth]{figures/3chain-tps}
%    \caption{Throughput of 3-chain HotStuff for various committee sizes. The transaction and batch sizes are set to 512B and 500KB respectively.}
%    \label{fig:3chain-tps}
%\end{figure}


%-------------------------------------------------------------------------------
%\subsection{Our new 2-Chain HotStuff}
%-------------------------------------------------------------------------------

%\begin{figure}[t]
 %   \centering
%    \includegraphics[width=0.47\textwidth]{figures/2chain-tps}
%    \caption{Throughput of 2-chain HotStuff for various committee sizes. The transaction and batch sizes are set to 512B and 500KB respectively.}
%    \label{fig:2chain-tps}
%\end{figure}


==> sections/experiments/async.tex <==
%-------------------------------------------------------------------------------
%\subsection{Our Async Fallback}
%-------------------------------------------------------------------------------



==> sections/experiments/sync.tex <==
%-------------------------------------------------------------------------------
%\subsection{Our Sync Path}
%-------------------------------------------------------------------------------



==> sections/experiments/vaba.tex <==
%-------------------------------------------------------------------------------
%\subsection{The (2-Chain) VABA}
%-------------------------------------------------------------------------------



==> sections/illustration_1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,640); %set diagram left start at 0, and has height of 640

%Shape: Rectangle [id:dp7152142976802189] 
\draw   (122.62,163.37) -- (151.28,163.37) -- (151.28,191.13) -- (122.62,191.13) -- cycle ;
%Shape: Rectangle [id:dp6908625380102904] 
\draw   (179.66,163.37) -- (208.32,163.37) -- (208.32,191.13) -- (179.66,191.13) -- cycle ;
%Shape: Rectangle [id:dp005329731199473997] 
\draw   (236.7,163.37) -- (265.36,163.37) -- (265.36,191.13) -- (236.7,191.13) -- cycle ;
%Shape: Diamond [id:dp3509423622564831] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (165.4,172.16) -- (168.96,177.15) -- (165.4,182.14) -- (161.83,177.15) -- cycle ;
%Straight Lines [id:da9470213255367586] 
\draw    (151.49,177.15) -- (180.01,177.15) ;
%Shape: Diamond [id:dp6126481552754586] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (222.44,172.16) -- (226,177.15) -- (222.44,182.14) -- (218.87,177.15) -- cycle ;
%Straight Lines [id:da5662876359446167] 
\draw    (208.53,177.15) -- (237.05,177.15) ;
%Shape: Diamond [id:dp24628558155779778] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (279.48,172.16) -- (283.04,177.15) -- (279.48,182.14) -- (275.91,177.15) -- cycle ;
%Straight Lines [id:da42541381859899663] 
\draw    (265.57,177.15) -- (293.38,177.15) ;
%Shape: Rectangle [id:dp9321568003011265] 
\draw   (64.86,163.37) -- (93.53,163.37) -- (93.53,191.13) -- (64.86,191.13) -- cycle ;
%Shape: Diamond [id:dp622806433737183] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (107.64,172.16) -- (111.21,177.15) -- (107.64,182.14) -- (104.08,177.15) -- cycle ;
%Straight Lines [id:da6615068728739755] 
\draw    (93.74,177.15) -- (122.26,177.15) ;
%Shape: Rectangle [id:dp08603854070851513] 
\draw   (179.87,21.12) -- (208.53,21.12) -- (208.53,48.88) -- (179.87,48.88) -- cycle ;
%Shape: Rectangle [id:dp865095487196669] 
\draw   (236.91,21.12) -- (265.57,21.12) -- (265.57,48.88) -- (236.91,48.88) -- cycle ;
%Straight Lines [id:da210007428517347] 
\draw    (111.21,177.15) -- (179.59,34.48) ;
%Shape: Diamond [id:dp3495421045482563] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (222.65,29.92) -- (226.22,34.91) -- (222.65,39.9) -- (219.09,34.91) -- cycle ;
%Straight Lines [id:da14140633146529247] 
\draw    (208.75,34.91) -- (237.27,34.91) ;
%Shape: Diamond [id:dp7830199847146715] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (279.69,29.92) -- (283.26,34.91) -- (279.69,39.9) -- (276.13,34.91) -- cycle ;
%Straight Lines [id:da9458735130692291] 
\draw    (265.79,34.91) -- (293.59,34.91) ;
%Shape: Rectangle [id:dp13825090177928234] 
\draw   (179.8,92.26) -- (208.46,92.26) -- (208.46,120.02) -- (179.8,120.02) -- cycle ;
%Shape: Rectangle [id:dp8967902778636039] 
\draw   (236.84,92.26) -- (265.5,92.26) -- (265.5,120.02) -- (236.84,120.02) -- cycle ;
%Straight Lines [id:da4118880850755393] 
\draw    (179.8,106.31) -- (168.96,177.15) ;
%Shape: Diamond [id:dp9835340339593011] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (222.58,101.05) -- (226.14,106.04) -- (222.58,111.03) -- (219.01,106.04) -- cycle ;
%Straight Lines [id:da7529994633464869] 
\draw    (208.68,106.04) -- (237.2,106.04) ;
%Shape: Diamond [id:dp7098437020108355] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (279.62,101.05) -- (283.19,106.04) -- (279.62,111.03) -- (276.06,106.04) -- cycle ;
%Straight Lines [id:da9174539594145732] 
\draw    (265.72,106.04) -- (293.52,106.04) ;
%Straight Lines [id:da9316427426277947] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (222.69,53.69) -- (222.69,79.89) ;
%Shape: Brace [id:dp7341277811026983] 
\draw   (178.73,210.24) .. controls (178.73,214.91) and (181.06,217.24) .. (185.73,217.24) -- (229.87,217.24) .. controls (236.54,217.24) and (239.87,219.57) .. (239.87,224.24) .. controls (239.87,219.57) and (243.2,217.24) .. (249.87,217.24)(246.87,217.24) -- (294,217.24) .. controls (298.67,217.24) and (301,214.91) .. (301,210.24) ;
%Shape: Brace [id:dp20816848980598657] 
\draw   (311.68,175.41) .. controls (316.35,175.41) and (318.68,173.08) .. (318.68,168.41) -- (318.68,115.89) .. controls (318.68,109.22) and (321.01,105.89) .. (325.68,105.89) .. controls (321.01,105.89) and (318.68,102.56) .. (318.68,95.89)(318.68,98.89) -- (318.68,43.37) .. controls (318.68,38.7) and (316.35,36.37) .. (311.68,36.37) ;
%Shape: Brace [id:dp11492854599064128] 
\draw   (20.84,210.59) .. controls (20.84,215.26) and (23.17,217.59) .. (27.84,217.59) -- (75.01,217.59) .. controls (81.68,217.59) and (85.01,219.92) .. (85.01,224.59) .. controls (85.01,219.92) and (88.34,217.59) .. (95.01,217.59)(92.01,217.59) -- (142.18,217.59) .. controls (146.85,217.59) and (149.18,215.26) .. (149.18,210.59) ;
%Straight Lines [id:da2277902482946712] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (64.65,177.26) -- (29,177.26) ;
%Shape: Rectangle [id:dp9183290152683508] 
\draw   (347.95,163.51) -- (376.61,163.51) -- (376.61,191.27) -- (347.95,191.27) -- cycle ;
%Shape: Rectangle [id:dp6771515880641845] 
\draw   (404.99,163.51) -- (433.65,163.51) -- (433.65,191.27) -- (404.99,191.27) -- cycle ;
%Shape: Diamond [id:dp9442643783790896] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (390.73,172.3) -- (394.29,177.3) -- (390.73,182.29) -- (387.16,177.3) -- cycle ;
%Straight Lines [id:da4246508108176754] 
\draw    (376.82,177.3) -- (405.34,177.3) ;
%Shape: Diamond [id:dp11809975058192324] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (447.77,172.3) -- (451.33,177.3) -- (447.77,182.29) -- (444.2,177.3) -- cycle ;
%Straight Lines [id:da9072082763029177] 
\draw    (433.86,177.3) -- (461.67,177.3) ;
%Straight Lines [id:da8989921489486599] 
\draw    (293.52,106.04) -- (347.73,177.65) ;
%Shape: Brace [id:dp18531096972388283] 
\draw   (336.68,210.38) .. controls (336.68,215.05) and (339.01,217.38) .. (343.68,217.38) -- (390.85,217.38) .. controls (397.52,217.38) and (400.85,219.71) .. (400.85,224.38) .. controls (400.85,219.71) and (404.18,217.38) .. (410.85,217.38)(407.85,217.38) -- (458.02,217.38) .. controls (462.69,217.38) and (465.02,215.05) .. (465.02,210.38) ;
%Straight Lines [id:da6121099077131795] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (222.83,125.78) -- (222.83,151.98) ;

% Text Node
\draw (172.14,225.95) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {$\displaystyle n$ f-chains, \\built by each \\replica};
% Text Node
\draw (15.95,228.32) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {steady state};
% Text Node
\draw (336.15,-0.43) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {once $\displaystyle n-f$ f-chain \\complete, \ select \\one from $\displaystyle n$ chains\\randomly};
% Text Node
\draw (336.75,224.09) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {steady state \\continues from the \\selected f-chain};


\end{tikzpicture}

==> sections/illustration_2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,517); %set diagram left start at 0, and has height of 517

%Shape: Rectangle [id:dp7890533729755063] 
\draw   (169.96,79.51) -- (203.35,79.51) -- (203.35,111.85) -- (169.96,111.85) -- cycle ;
%Shape: Rectangle [id:dp8058947703644723] 
\draw   (236.4,79.51) -- (269.79,79.51) -- (269.79,111.85) -- (236.4,111.85) -- cycle ;
%Shape: Rectangle [id:dp5304722945812508] 
\draw   (343.88,79.51) -- (377.27,79.51) -- (377.27,111.85) -- (343.88,111.85) -- cycle ;
%Shape: Diamond [id:dp9169733555271671] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (219.79,89.75) -- (223.95,95.57) -- (219.79,101.38) -- (215.64,95.57) -- cycle ;
%Straight Lines [id:da20382205833144318] 
\draw    (203.6,95.57) -- (236.82,95.57) ;
%Shape: Diamond [id:dp7713914047543382] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (286.24,89.75) -- (290.39,95.57) -- (286.24,101.38) -- (282.09,95.57) -- cycle ;
%Straight Lines [id:da3844984263310154] 
\draw    (270.04,95.57) -- (344,95.57) ;
%Straight Lines [id:da22228183188182316] 
\draw    (285.82,84.77) -- (285.82,61.85) ;
\draw [shift={(285.82,59.85)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1481630048928959] 
\draw    (219.38,84.77) -- (219.38,61.85) ;
\draw [shift={(219.38,59.85)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp9268625520427971] 
\draw   (102.68,79.51) -- (136.07,79.51) -- (136.07,111.85) -- (102.68,111.85) -- cycle ;
%Shape: Diamond [id:dp1958700100901014] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (152.52,89.75) -- (156.67,95.57) -- (152.52,101.38) -- (148.36,95.57) -- cycle ;
%Straight Lines [id:da46311620533380626] 
\draw    (136.32,95.57) -- (169.54,95.57) ;
%Straight Lines [id:da6064290575992173] 
\draw    (152.1,84.77) -- (152.1,61.85) ;
\draw [shift={(152.1,59.85)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Brace [id:dp7215923084371985] 
\draw   (165.91,163.67) .. controls (165.94,168.34) and (168.28,170.66) .. (172.95,170.63) -- (223.85,170.32) .. controls (230.52,170.28) and (233.86,172.59) .. (233.89,177.26) .. controls (233.86,172.59) and (237.18,170.24) .. (243.85,170.2)(240.85,170.22) -- (294.75,169.89) .. controls (299.42,169.86) and (301.74,167.51) .. (301.71,162.84) ;
%Shape: Brace [id:dp38980865321725755] 
\draw   (350.07,161.84) .. controls (350.07,166.51) and (352.4,168.84) .. (357.07,168.84) -- (381.81,168.84) .. controls (388.48,168.84) and (391.81,171.17) .. (391.81,175.84) .. controls (391.81,171.17) and (395.14,168.84) .. (401.81,168.84)(398.81,168.84) -- (426.54,168.84) .. controls (431.21,168.84) and (433.54,166.51) .. (433.54,161.84) ;
%Shape: Brace [id:dp010036188492620335] 
\draw   (65.31,163.26) .. controls (65.31,167.93) and (67.64,170.26) .. (72.31,170.26) -- (97.04,170.26) .. controls (103.71,170.26) and (107.04,172.59) .. (107.04,177.26) .. controls (107.04,172.59) and (110.37,170.26) .. (117.04,170.26)(114.04,170.26) -- (141.78,170.26) .. controls (146.45,170.26) and (148.78,167.93) .. (148.78,163.26) ;
%Straight Lines [id:da8282524810587044] 
\draw [line width=0.75]  [dash pattern={on 0.84pt off 2.51pt}]  (66.55,95.57) -- (102.27,95.57) ;
%Shape: Circle [id:dp403292123226882] 
\draw   (320.2,95.57) .. controls (320.2,92.36) and (322.81,89.75) .. (326.02,89.75) .. controls (329.23,89.75) and (331.83,92.36) .. (331.83,95.57) .. controls (331.83,98.78) and (329.23,101.38) .. (326.02,101.38) .. controls (322.81,101.38) and (320.2,98.78) .. (320.2,95.57) -- cycle ;
%Straight Lines [id:da5541775772785338] 
\draw    (326.43,83.94) -- (326.43,72.03) ;
\draw [shift={(326.43,70.03)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Diamond [id:dp42606973756108824] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (393.3,89.34) -- (397.45,95.15) -- (393.3,100.96) -- (389.14,95.15) -- cycle ;
%Straight Lines [id:da5205872719892832] 
\draw    (377.1,95.15) -- (410.32,95.15) ;

% Text Node
\draw (186.65,95.68) node  [font=\large]  {$\overline{B}_{1,L}$};
% Text Node
\draw (360.57,95.68) node  [font=\large]  {$B_{r_{cur}}$};
% Text Node
\draw (173.54,35.9) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {height-$\displaystyle 1$ $\displaystyle \overline{qc}$};
% Text Node
\draw (159.4,117.93) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {round $\displaystyle r$\\height $\displaystyle 1$};
% Text Node
\draw (119.38,95.68) node  [font=\large]  {$B_{r'}$};
% Text Node
\draw (122.11,34.41) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle qc_{high}$};
% Text Node
\draw (92.95,119.79) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {round $\displaystyle r'$};
% Text Node
\draw (321.74,119.37) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {round $\displaystyle r_{cur} =r+2$};
% Text Node
\draw (156.5,179.73) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {f-chain of replica $\displaystyle L$};
% Text Node
\draw (352.23,180.51) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {back to steady state};
% Text Node
\draw (275.4,7.28) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle 2f+1$ height-2 $\displaystyle \overline{qc}$ to \\trigger leader election};
% Text Node
\draw (217.68,117.93) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {round $\displaystyle r+1$\\height $\displaystyle 2$};
% Text Node
\draw (253.1,95.68) node  [font=\large]  {$\overline{B}_{2,L}$};
% Text Node
\draw (27.99,180.59) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {steady state};
% Text Node
\draw (311.01,52.36) node [anchor=north west][inner sep=0.75pt]  [font=\Large] [align=left] {$\displaystyle qc_{coin}$};


\end{tikzpicture}
